Algorithms for Game Metrics

Simulation and bisimulation metrics for stochastic systems provide a quantitative generalization of the classical simulation and bisimulation relations. These metrics capture the similarity of states with respect to quantitative specifications written in the quantitative {\mu}-calculus and related probabilistic logics. We first show that the metrics provide a bound for the difference in long-run average and discounted average behavior across states, indicating that the metrics can be used both in system verification, and in performance evaluation. For turn-based games and MDPs, we provide a polynomial-time algorithm for the computation of the one-step metric distance between states. The algorithm is based on linear programming; it improves on the previous known exponential-time algorithm based on a reduction to the theory of reals. We then present PSPACE algorithms for both the decision problem and the problem of approximating the metric distance between two states, matching the best known algorithms for Markov chains. For the bisimulation kernel of the metric our algorithm works in time O(n^4) for both turn-based games and MDPs; improving the previously best known O(n^9\cdot log(n)) time algorithm for MDPs. For a concurrent game G, we show that computing the exact distance between states is at least as hard as computing the value of concurrent reachability games and the square-root-sum problem in computational geometry. We show that checking whether the metric distance is bounded by a rational r, can be done via a reduction to the theory of real closed fields, involving a formula with three quantifier alternations, yielding O(|G|^O(|G|^5)) time complexity, improving the previously known reduction, which yielded O(|G|^O(|G|^7)) time complexity. These algorithms can be iterated to approximate the metrics using binary search.

==> abstract.tex <==
Simulation and bisimulation metrics for stochastic systems provide a
quantitative generalization of the classical simulation and
bisimulation relations. 
These metrics capture the similarity of states with respect to
quantitative specifications written in the quantitative $\mu$-calculus
and related probabilistic logics.
%We first show that the metrics provide a bound also for the 
%difference in {\em long-run average\/} and {\em discounted average\/}
%behavior across states, indicating that the metrics can be used both
%in system verification, and in performance evaluation. 

We present algorithms for computing the metrics on Markov
decision processes (MDPs), turn-based stochastic games, and concurrent
games.  
For turn-based games and MDPs, we provide a polynomial-time algorithm
for the computation of the one-step metric distance between states. 
The algorithm is based on linear programming; it improves on the
previous known exponential-time algorithm based on a reduction to the theory of
reals.
We then present PSPACE algorithms for both the decision problem and the
problem of approximating the metric distance between two states,
%
%for the metric
%distance between two states, and to approximately compute the metric distance 
%between two states,
%
%%%The one-step operator gives a polynomial space procedure to approximately compute
%%the metric between two states, 
matching the best known algorithms for Markov chains. 
For the bisimulation kernel of the metric, which corresponds to probabilistic
bisimulation, our algorithm works in time $\calo(n^4)$ for both 
turn-based games and MDPs; improving the previously best known 
$\calo(n^9\cdot\log(n))$ time algorithm for MDPs. 

For a concurrent game $G$, we show that computing the exact distance
between states is at least as hard as computing the value of
concurrent reachability games and
the square-root-sum problem in computational geometry.
We show that checking whether the metric distance is bounded by a 
rational $r$, can be accomplished via a reduction to the theory of 
real closed fields, involving a formula with three quantifier 
alternations, yielding $\calo(|G|^{\calo(|G|^5)})$ time 
complexity, improving the previously known reduction, which yielded  
$\calo(|G|^{\calo(|G|^7)})$ time complexity.  
These algorithms can be iterated to approximate the metrics using
binary search. 


==> games.tex <==
\section{Algorithms for concurrent games}
\label{sec-conc-algos}
%
We first show that the complexity of computing the undiscounted
a priori simulation metric is at least as hard as concurrent 
reachability, which is not known to be in PSPACE.
We then present algorithms based on a decision procedure for
the theory of reals.

\input{reduction}

\smallskip\noindent{\bf Algorithms for the one-step a priori metric 
distance.}
%
We now look at an algorithm for the undiscounted a priori game 
simulation metric.
The case for the discounted metric is similar.
Since the a priori metric is reciprocal, we consider the 
player~1 distance; the player~2 distance will be the same.
Given a $\delta \in (0, 1)$, and states $s, t \in S$, we answer 
the question $\metr{s \priosim t} > \delta$.
We define the predicate $\IsDistribution(x, \mov)$ that checks 
if a variable $x$ is a probability distribution with support
$\mov$.
%
\[
\IsDistribution(x,\mov) =
\bigwedge_{a \in \mov} x(a) \ge 0 \; \wedge
\bigwedge_{a \in \mov} x(a) \le 1 \; \wedge
\sum_{a \in \mov} x(a) = 1
\]
%
We introduce the predicate $\IsValidValuation(k, d)$, which 
checks if a variable $k$ is a valid valuation bounded by
the distance $d$.
%
\begin{align*}
& \IsValidValuation(k, d, S) = \\
& \quad
\bigwedge_{u \in S} k(u) \ge 0 \; \wedge
\bigwedge_{u \in S} k(u) \le 1 \; \wedge
\bigwedge_{u, v \in S} (k(u) - k(v) \le d(u, v)
\end{align*}
%
We introduce the following predicate that checks if the
propositional distance between two states $s$ and $t$ is
at least $\delta$.
%
\[
\PropDistance(s, t, \vars, \delta) =
\bigvee_{p \in \vars} (\int{p}(s) - \int{p}(t)) > \delta
\]
%
We now introduce the predicate $\ExactOneStepDistance(s, t, G, 
\delta)$, that checks if the exact one-step a priori distance 
between $s$ and $t$ is at least $\delta$.
%
\begin{align*}
& \ExactOneStepDistance(s, t, d, G, \delta) = \\
& \quad
\bigl(
\PropDistance(s, t, \vars, \delta) > \delta
\bigr) \; \vee \\
& \quad
\forall_{k} . \forall_{x_1} . \exists_{y_1} .
\bigl[
\bigwedge_{c \in \mov_2(t)} 
\bigl(
\exists_{x_2} .
(\sum_{u \in S} (\trans(s, x_1, x_2)(u) \; k(u) -
 \trans(t, y_1, c)(u) \; k(u))) > \delta) \; \wedge \\
& \quad
\IsValidValuation(k, d) \wedge
\IsDistribution(x_1, \mov_1(s)) \wedge
\IsDistribution(y_1, \mov_1(t)) \; \wedge \\
& \quad
\IsDistribution(x_2, \mov_2(s))
\bigr) 
\bigr]
\end{align*}
%
We note that $\ExactOneStepDistance$ is a formula with one 
quantifier alternation and hence can be decided using a decision 
procedure for the theory or reals with one quantifier alternation; 
which is known to be in EXPTIME.
The formula reduces the number of quantifier alternations from
$3$ to $1$ in the case of the a priori game simulation metric.
\mynote{I am here. For the exact distance in the limit, the above
decision procedure is not immediately useful as we need to get
the distance updated for the next iteration. I need to figure out
how. For the kernel of the a posteriori metric, we are fine as
we only need to check for a match in distributions induced over
states.}

From Theorem~\ref{theo-metrics-diff} we know that the a 
posteriori game simulation metric is an upper bound on the a
priori metric. 

We define the following predicate for the a priori kernel:

\begin{align*}
&\APrioriKernel(s, t, G, d, r, \delta) =
\forall k . \forall x_1 . \exists y_1 .
\biggl\{
\bigwedge_{c \in \mov_2(t)}
\biggl[
\exists x_2 . \\
& \quad
\biggl(
\sum_{u \in S}\trans(t, y_1, c)(u) \; k(u) \ge 
\sum_{u \in S}\trans(s, x_1, x_2)(u) \; k(u)
\biggr)
\biggr]
\biggr\} \wedge \\
& \quad
\IsDistribution(x_2, \mov_2(s)) \wedge
\IsDistribution(y_1, \mov_1(t)) \wedge
\IsDistribution(x_1, \mov_1(s)) \wedge
\IsValidValuation(k, d)
\end{align*}

